Where to Begin? On the Impact of Pre-Training and Initialization in Federated Learning

An oft-cited challenge of federated learning is the presence of heterogeneity. \emph{Data heterogeneity} refers to the fact that data from different clients may follow very different distributions. \emph{System heterogeneity} refers to client devices having different system capabilities. A considerable number of federated optimization methods address this challenge. In the literature, empirical evaluations usually start federated training from random initialization. However, in many practical applications of federated learning, the server has access to proxy data for the training task that can be used to pre-train a model before starting federated training. Using four standard federated learning benchmark datasets, we empirically study the impact of starting from a pre-trained model in federated learning. Unsurprisingly, starting from a pre-trained model reduces the training time required to reach a target error rate and enables the training of more accurate models (up to 40\%) than is possible when starting from random initialization. Surprisingly, we also find that starting federated learning from a pre-trained initialization reduces the effect of both data and system heterogeneity. We recommend future work proposing and evaluating federated optimization methods to evaluate the performance when starting from random and pre-trained initializations. This study raises several questions for further work on understanding the role of heterogeneity in federated optimization. \footnote{Our code is available at: \url{https://github.com/facebookresearch/where_to_begin}}

==> [ICLR] Where to begin_/abstract.tex <==
\begin{abstract}
An oft-cited challenge of federated learning is the presence of heterogeneity. \emph{Data heterogeneity} refers to the fact that data from different clients may follow very different distributions. \emph{System heterogeneity} refers to client devices having different system capabilities. A considerable number of federated optimization methods address this challenge. In the literature, empirical evaluations usually start federated training from random initialization. However, in many practical applications of federated learning, the server has access to proxy data for the training task that can be used to pre-train a model before starting federated training. Using four standard federated learning benchmark datasets, we empirically study the impact of starting from a pre-trained model in federated learning. Unsurprisingly, starting from a pre-trained model reduces the training time required to reach a target error rate and enables the training of more accurate models (up to 40\%) than is possible when starting from random initialization. Surprisingly, we also find that starting federated learning from a pre-trained initialization reduces the effect of both data and system heterogeneity. We recommend future work proposing and evaluating federated optimization methods to evaluate the performance when starting from random and pre-trained initializations. This study raises several questions for further work on understanding the role of heterogeneity in federated optimization.
\footnote{Our code is available at: \url{https://github.com/facebookresearch/where_to_begin}}
\end{abstract}

==> [ICLR] Where to begin_/acks.tex <==
\section*{Acknowledgement}
We would like to thank Akshat Shrivastava, Hongyuan Zhan, Daniel Lazar, and Ashish Shenoy for their helpful discussions at various stages of this work.

==> [ICLR] Where to begin_/conclusion.tex <==
\section{Conclusion and Limitations}
% \label{sec:limitations}
\label{sec:conclusion}
\textbf{Limitations.} Depending on the application, it may not be possible to get public data, in which case random initialization may be the only option. Nevertheless, we believe there is sufficient prevalence and importance of applications where public data is available for this study to be of broad interest. When public data is available, it may not necessarily reflect the distribution of all users in the population. Consequently, pre-training using public data may introduce bias, which warrants further study, including methods to detect and mitigate such bias. Moreover, we only consider one warm-start initialization strategy: supervised pre-training. Several other possibilities are worth investigating, including meta-learning the warm-start initialization and self-supervised pre-training. 

% Another interest direction is to study shared presentation in FL where heterogeneous data distributed across tasks may share a common representation despite having different labels \cite{}

\textbf{Conclusion.} In this paper, we present a thorough empirical analysis of initialization on federated learning by evaluating it on twelve federated learning algorithms across four vision and text tasks. We find that pre-training on public data can recover most of the accuracy drop from heterogeneity. We show that client updates starting from pre-trained weights have higher cosine similarity, which explains why initializing with pre-trained weights can speed up convergence and achieve high accuracy even in heterogeneous settings. We further show that using simple \sgd locally can be as good as other local optimizers. 


==> [ICLR] Where to begin_/experiments.tex <==
\section{Experimental Setup}
\label{sec:experiments}
% Next, we describe the experimental setup used to evaluate how initialization impacts the performance of federated optimization methods.  
% We consider 15 possible combinations of \serveropt and \clientopt across four tasks. 
% Details about the experiments, hyper-parameters, and models are in Appendix~\ref{sec:appendix_exp}.

\subsection{Datasets, Models, and Tasks}
We experiment on four FL benchmark datasets: CIFAR-10, FEMNIST, Stack Overflow, and Reddit. All datasets have a natural non-IID partitioning of the data except for CIFAR-10, which we partition using a Dirichlet distribution with $\alpha \in [0.1, 1.0, 10]$. We train Squeezenet and ResNet18 models for CIFAR-10 and FEMNIST, and DistilGPT2 and CharLM models for Stackoverflow and Reddit pushift.io. See Appendix~\ref{sec:appendix_dataset_model} for additional information. We run each experiment with three different seeds and report the average. We tune client and server learning rates $\eta_{\ell}$ and $\eta_g$, and the proximal penalty parameter $\mu$ for \textsc{FedProx} with a hyperparameter sweep. Each client update runs one local epoch with fixed batch size per task, and we perform 1050 rounds of training for Stackoverflow, 1000 rounds of training for CIFAR-10, and 1082 training rounds for FEMNIST. For additional implementation details, see Appendix~\ref{sec:appendix_imple}. We use the open-source federated learning simulation framework FLSim~\cite{flsim}.


% To facilitate comparing with other work in the literature, we experiment on four standard FL benchmark datasets: CIFAR-10 \citep{cifar10}, Federated EMNIST-62 (FEMNIST) \citep{cohen2017emnist, leaf}, Stack Overflow \citep{stackoverflow} and Reddit \citep{leaf}.

% \paragraph{Non-IID data partitioning.} Unless otherwise mentioned, we use non-independent and identically distributed (non-IID) splits of data across clients to mimic data heterogeneity commonly observed in practice. 
% CIFAR-10 is an image classification task with 10 classes. We generate 500 non-IID clients using a Dirichlet distribution with $\alpha = 0.1$, using the approach described in \citet{fedavgm}.
% The FEMNIST task is to classify images of characters. We use the federated version where characters are partitioned by their author~\cite{leaf}.
% For Stack Overflow, the data at each client corresponds to the questions and answers of one user on stackoverflow.com, and we train a language model for a next-word-prediction task. For Reddit, the data at each client is text from posts and comments of a Reddit user, and we train a language model for next-word-prediction for this dataset~\cite{leaf}. 

% % For CelebA, we partition data across clients by taking each client to be one celebrity who uploaded the images of themselves. The taks is to train a model for a binary smile classification task (smiling vs not smiling).

% \paragraph{IID data partitioning.} To understand the effect of data heterogeneity, we run some experiments using an IID partition of data across clients. In this case we first group the entire training set (from all clients), randomly permute it, and then partition it evenly across the same number of clients. 

% \paragraph{Models.} For CIFAR-10 and FEMNIST, we use the Squeezenet~\citep{squeezenet} and ResNet18~\citep{resnet} models, with batch norm replaced with group norm as commonly done in FL literature~\citep{adaptive-fl-optimization, hsieh_quagmire}. For Stackoverflow and Reddit, we use the DistilGPT2~\citep{distilgpt2} and CharLM~\citep{char_lm} models. For additional information about the datasets and models, see Appendix~\ref{sec:appendix_dataset_model}. 


\subsection{Initialization Strategies}
We consider two initialization strategies: random initialization and supervised pre-training. 

\textbf{Random initialization.} Most prior federated optimization works use random weights to initialize the model. We can use the same random initialization strategies used in the standard (centralized) training of deep networks for each model~\citep{squeezenet, distilgpt2, resnet, char_lm}.

\textbf{Supervised pre-training.} In many FL applications, pre-training can be done on a large non-private proxy dataset available at the server. To facilitate easily reproducing our results, we use publicly available pre-trained models or pre-train on public data. For tasks using Squeezenet and ResNet18, we use the version of the model pre-trained on ImageNet, available in the PyTorch Torchvision library.\footnote{\url{https://github.com/pytorch/vision}} For tasks using DistilGPT2, we use the model weights provided in the HuggingFace library that has been distilled from a pre-trained GPT2,\footnote{\url{https://huggingface.co/distilgpt2}} and for tasks using CharLM, we pre-train the model on WikiText-103~\citep{wikitext103} (see Appendix \ref{sec:char_lm_pre} for details). 

% Supervised pre-training is just one possibility, and we leave the investigation of other pre-training strategies (e.g., self-supervised pre-training and meta-learning) as future work; see Section~\ref{sec:conclusion}.

\subsection{Algorithms}
\label{sec:algorithms}
% We compare federated training with five \clientopt strategies: (\textbf{SGD}) standard SGD updates, (\textbf{\FedProx}) style local updates to reduce client drift, (\textbf{\FedNova}) style updates and aggregation to compensate for data imbalance, (\textbf{\mimelite}) that makes use of an optimizer state from the server, and (\textbf{GD}) full-batch gradient updates. 

% We consider three \serveropt strategies: (\textbf{FedAvg}) the server updates the global model using stochastic gradient descent; when \clientopt is also SGD, this is equivalent to \textsc{FedAvg}~\citep{google-fedavg}, (\textbf{FedAvgM}) the server updates the global model using SGD with momentum; when \clientopt is SGD, this is equivalent to \textsc{FedAvgM}~\citep{fedavgm}, and (\textbf{FedAdam}) Adam optimizer, the server updates the global model using the Adam optimizer; when \clientopt is SGD, this is equivalent to \textsc{FedAdam}~\citep{adaptive-fl-optimization}. \textbf{\textsc{FedSGD}} is obtained when \clientopt is GD and \serveropt is SGD with $\eta_c = 1$ and $E=1$. We focus on these choices because they are widely used and represent a diverse set of options for cross-device federated training at scale.

We compare federated training with five different \clientopt strategies: 
\begin{description}
\item[SGD] clients perform standard stochastic gradient descent updates;
\item[Proximal~\citep{fedprox}] clients perform \FedProx-style local updates; \FedProx was originally proposed to reduce client drift due to heterogeneity;
\item[Normalized Averaging~\citep{fednova}] clients use \FedNova-style updates and aggregation to compensate for data imbalance across clients;
\item[\mimelite~\citep{karimireddy2021mime}] clients make use of an optimizer state (e.g., momentum buffer) from the server during local updates to reduce drift due to data heterogeneity;
\item[GD] clients perform full-batch gradient updates; in this case, the update $\Delta_i^t$ returned to the server is a full-batch gradient on client $i$'s local training set evaluated at model parameters $x^{t-1}$.
\end{description}

At the server, we consider three strategies for \serveropt. In all strategies, the server treats the averaged update $\Delta^t$ as a gradient.
\begin{description}
\item[SGD] the server updates the global model using stochastic gradient descent; when \clientopt is also SGD, this is equivalent to \textsc{FedAvg}~\citep{google-fedavg}.

\item[SGD with momentum] the server updates the global model using SGD with momentum; when \clientopt is SGD, this is equivalent to \textsc{FedAvgM}~\citep{fedavgm}.

\item[Adam] the server updates the global model using the Adam optimizer; when \clientopt is SGD, this is equivalent to \textsc{FedAdam}~\citep{adaptive-fl-optimization}.
\end{description}

The method commonly referred to as \textsc{FedSGD}~\citep{mcmahan2016communication} is obtained when \clientopt is full-batch gradient descent (GD) and \serveropt is SGD, with $\eta_c = 1$ and $E=1$.

We focus on the above choices for \clientopt and \serveropt because they are reflective of the most widely-cited federated optimization methods, and they also represent a diverse set of possible choices available to the practitioner seeking to deploy cross-device federated training at scale.

\subsection{Implementation and Tuning}
We use three different seeds and report the average of each experiment. Hyperparameter tuning is done for each algorithm, model, and dataset, with parameters including client and server learning rates $\eta_{\ell}$ and $\eta_g$, and the proximal penalty parameter $\mu$ for \textsc{FedProx}. Unless otherwise specified, we perform one local epoch with fixed batch size per task for each client update. For Stackoverflow, we perform 1050 training rounds. For CIFAR-10, we perform 1000 training rounds. For FEMNIST, we perform 1082 training rounds. Our experiments are implemented using the open-source federated learning simulation framework FLSim~\cite{flsim}. Further implementation details can be found in Appendix~\ref{sec:appendix_imple}.

% To facilitate comparing with other work in the literature, we experiment on four standard FL benchmark datasets: CIFAR-10 \citep{cifar10}, Federated EMNIST-62 (FEMNIST) \citep{cohen2017emnist, leaf}, Stack Overflow \citep{stackoverflow} and Reddit pushift.io \citep{leaf}. All datasets have a natural non-IID partitioning of the data except for CIFAR-10, for which we use the Dirichlet allocation approach of~\cite{fedavgm} with parameter $0.1$ to partition data across 50 users. For CIFAR-10 and FEMNIST, we train Squeezenet~\citep{squeezenet} and ResNet18~\citep{resnet} models, replacing batch norm with group norm ~\citep{adaptive-fl-optimization, hsieh_quagmire}. For Stackoverflow and Reddit pushift.io, we use the DistilGPT2~\citep{distilgpt2} and CharLM~\citep{char_lm} models. For additional information about the datasets and models, see Appendix~\ref{sec:appendix_dataset_model}. 

==> [ICLR] Where to begin_/intro.tex <==
\section{Introduction}
\label{sec:intro}
\emph{Federated learning} (FL) has emerged as a popular distributed machine learning paradigm for privately training a shared model across many participants. At the same time, the training data never leaves the participant's devices. This paper empirically investigates the impact of model initialization on federated optimization methods. Previous empirical evaluations of FL methods start federated training from a randomly initialized model. Transfer learning from pre-trained models has become common practice in natural language processing~\cite{gpt2,devlin2018bert} and computer vision~\cite{he2019rethinking,vit}, yielding state-of-the-art results on many tasks and enabling faster model convergence in the centralized setting. Although public proxy data is available at the server in many applications, few prior works studied the impact of starting federated training from a pre-trained model.

In cross-device FL~\citep{fl-survey}, the primary setting considered in this paper, a central server coordinates many client devices (possibly in hundreds of millions). Each device possesses a local dataset, and the data at different devices follow different distributions, leading to the \emph{data heterogeneity} challenge~\citep{fl-survey}. Moreover, client devices have different system capabilities, leading to \emph{system heterogeneity}. Finally, devices communicate with the server over low-bandwidth communication links making the performance bottleneck.

The predominant approach to federated training builds on local update methods such as \textsc{FedAvg}~\citep{google-fedavg}, where a device performs several local updates (e.g., one epoch of SGD on their local training set) before transmitting an update to the server. Although this reduces communication overhead, it can also exacerbate data heterogeneity. Several approaches have been proposed to address this challenge~\citep{fedprox,fedavgm,adaptive-fl-optimization,fednova,SCAFFOLD,karimireddy2021mime,zhang2021fedpd,acar2021feddyn}. However, few prior works examine the impact of initialization on federated training. 

\paragraph{Contributions.} In this work, we consider the question: {\it How does model initialization (random or pre-trained) impact the behavior of federated optimization methods?} We perform an extensive empirical study, comparing 15 variations of federated optimization methods on four commonly-used FL benchmark datasets. Our study reveals three key findings:
\begin{enumerate}
    \item Although optimizers designed to address heterogeneity typically lead to better performance when starting from a random initialization, when starting from a pre-trained model, we observe that (cf.~Fig.~\ref{fig:ranking}): (i) there is not as big a difference between optimizers in terms of accuracy after a fixed number of rounds, and (ii) using an adaptive optimizer at the server, such as \fedadam, is more important than using any method for addressing heterogeneity.

    \item Starting from a pre-trained model significantly reduces the difference between having non-IID vs. IID data for clients. Furthermore, when starting from a pre-trained model, the number of local epochs per round can be significantly increased without degrading the final accuracy.
    
    \item The initial loss is sometimes lower when starting from a random model. However, the largest Hessian eigenvalue (i.e., local Lipshitz constant or smoothness) is consistently smaller at initialization when starting from a pre-trained model compared to when starting from random initialization.
\end{enumerate}
Some of our empirical observations are consistent with existing FL theoretical convergence guarantees. Our findings also highlight that some aspects of FL are not captured with the existing theory, suggesting directions for future work.

Initializing FL with a pre-trained model can increase final model accuracy and reduce the number of rounds required to achieve a target accuracy. Pre-training leads to communication savings and reduces the overall training time. Figure \ref{fig:pretrained_vs_random} demonstrates the benefit of pre-training across several datasets (hyperparameters were tuned separately for each dataset--initialization pair; see Section~\ref{sec:experiments} for details of the experimental setup). 

\begin{figure*}[t]
     \centering
     \begin{minipage}[t]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/cifar_ranking_v2.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/so_ranking_v2.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/femnist_ranking_v2.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/reddit_ranking_v2.pdf}
     \end{minipage}
     \caption{We tested the accuracy of four datasets using random and pre-trained weights. We used solid lines for \sgd, dashed lines for \proximal, and dotted lines for \mimelite. The graph shows how the algorithm rankings changed between the random and pre-trained models. Although no single method is the best for all tasks, \fedadam with SGD for \clientopt performed consistently well when starting from a pre-trained model, especially for the larger language modeling tasks of Stack Overflow and Reddit.}
     \label{fig:ranking}
\end{figure*}
% \john{Update Figure \ref{fig:ranking} with different colors}

Our findings are reproducible using the open-source federated learning framework FLSim~\citep{flsim}. Informed by these findings, we present several recommendations for future research on federated optimization.

==> [ICLR] Where to begin_/intro_old.tex <==
\section{Introduction}
\label{sec:intro}
\emph{Federated learning} (FL) has emerged as a popular distributed machine learning paradigm for privately training a shared model across many participants while the training data never leaves the participant devices. Our focus in this work is on understanding the impact of model initialization on federated learning.

In cross-device FL~\citep{fl-survey}, the primary setting considered in this paper, a large number of client devices (possibly on the order of hundreds of millions) participate in training, which is coordinated by a server. It is impractical for all devices to participate at every step of training; instead, FL usually proceeds in rounds and a small subset of available devices participate in each round. Each device possesses a local dataset, and the data at different devices follow different distributions, leading to the \emph{data heterogeneity} challenge~\citep{fl-survey}. Moreover, devices communicate with the server over low-bandwidth, high-latency links, making communication overhead a major performance factor.

The predominant approach to federated training builds on local update methods such as \textsc{FedAvg}~\citep{google-fedavg}, where a device performs several local updates (e.g., one epoch of SGD on their local training set) before transmitting an update to the server. Although this reduces communication overhead, it can also exacerbate the data heterogeneity problem. Several approaches have been proposed to address this challenge~\citep{fedprox,fedavgm,adaptive-fl-optimization,fednova,SCAFFOLD,karimireddy2021mime,zhang2021fedpd,acar2021feddyn}.

\textbf{This paper empirically investigates the impact of model initialization on federated optimization methods.} Previous empirical evaluations of FL methods nearly always start federated training from a randomly initialized model. Transfer learning from pre-trained models has become common practice in natural language processing~\cite{gpt2,devlin2018bert} and computer vision~\cite{he2019rethinking,vit}, yielding state-of-the-art results on many tasks and enabling faster model convergence in the centralized setting. However, the impact of starting federated training from a pre-trained model has not been carefully studied, even though in many practical applications of FL there is public proxy data available for pre-training at the server.

\paragraph{Contributions.} In this work we consider the question:
\begin{center}
    \it How does model initialization (random, or pre-trained) impact \\the behavior of federated optimization methods?
\end{center}
Towards answering this question, we perform an extensive empirical study, comparing 15 variations of federated optimization methods on four commonly-used FL benchmark datasets. Our study reveals four key findings:
\begin{enumerate}
    % \item Federated optimization methods behave differently when initialized randomly versus from pre-trained weights (Section~\ref{sec:results_ranking}). \mike{Definitely rewrite this to be more specific; currently too vague or just not so surprising.}
    % \item \mike{Shouldn't the first point be about optimizers designed to address heterogeneity not being the best when starting from a pre-trained initialization?}
    \item Optimizers designed to address heterogeneity are not as effective when starting from pre-trained initialization. 
    % the effect of system and data heterogeneity is less of a problem when initializing federated optimization from a pre-trained solution.  \mike{Again, elaborate on exactly what ``less of a problem'' means here.}

    \item Starting from a pre-trained solution can close the gap between training on IID and non-IID data (Section~\ref{sec:results}). Moreover, the simple \sgd at the client outperforms more complex local-update methods in the pre-trained setting.
    
    \item Towards starting to explain this phenomenon, we observe that inter-device gradient/update diversity is higher for random initialized model at the beginning of training, and inter-device cosine similarity is higher when starting from a pre-trained model. (Section~\ref{sec:why_pretrain})
    
    \item When starting from a pre-trained solution, the client can afford to take more local steps to save on communications without hurting final accuracy. \john{Reword this finding}
    
    % Surprisingly, full-batch gradient descent, without any local steps, achieves performance competitive with other SoTA local-update methods from a pre-trained initialization. 

    % \mike{Maybe add something specifically about the performance of local-update methods vs those that don't use local updates (FedGD, ...)?}

\end{enumerate}
Our experiments also confirm what one might expect, that initializing FL with a pre-trained model can increase final model accuracy and reduce the number of rounds required to achieve a target accuracy, thereby saving communications and reducing the overall training time. This is evident in Figure~1 across several datasets (hyperparameters were tuned separately for each dataset--initialization pair; see Section~\ref{sec:experiments} for details of the experimental setup). 

\begin{figure*}[t]
     \centering
     \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/so_pre_ran.pdf}
     \end{minipage}
    \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/so_charlm_ran_pre.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.25\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/reddit_ran_pre.pdf}
     \end{minipage}
      \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/cifar_pre_ran.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/cifar_resnet_ran_pre.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.25\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/femnist_pre_ran.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.25\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/femnist_resnet_ran_pre.pdf}
     \end{minipage}
     \caption{While prior works ignore the importance of initialization, using pre-trained models should be the first step for any practical deployment to save on communication bandwidth and achieve high model accuracy. This figure shows the advantage of using a pre-trained model for four tasks. For Stack Overflow and Reddit, we use DistilGPT2 and CharLM. For CIFAR-10 and FEMNIST, we use SqueezeNet and ResNet18. }
     \label{fig:pretrained_vs_random}
\end{figure*}

Our findings are reproducible using the open-source federated learning framework FLSim~\cite{flsim}. Informed by these findings, we conclude by presenting several recommendations for future research on federated optimization.

==> [ICLR] Where to begin_/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> [ICLR] Where to begin_/prelim.tex <==
\section{Problem Formulation and the \fedopt framework}
\label{sec:prelim}


\begin{figure*}[t]
	\centering
    \begin{algorithm}[H]
        \begin{algorithmic}[1]
        \STATE {\bfseries Input:}  initial global model $x^0$, server and client step sizes $\eta_s$, $\eta_c$, local epochs $E$, rounds $T$
        \FOR{each round $t=1,\dots,T$}
            \STATE Server sends $x^{t-1}$ to all clients $i\in \mathcal{S}^t$.
            \FOR{each client $i\in \mathcal{S}^t$ in parallel}
                \STATE Initialize local model $y^0_i \leftarrow x^{t-1}$.
                \STATE Each client performs $E$ epochs of local updates via $y^{k+1}_i = \clientopt(y^k_i, F_i, \eta_c)$. Let $y^E_i$ denote the result after performing $E$ epochs of local updates.
                \STATE After local training, client $i$ sends $\Delta^t_i = x^{t-1} - y^E_i$ to the server.
            \ENDFOR
            \STATE Server computes aggregate update $\Delta^t = \frac{1}{|\mathcal{S}^t|} \sum_{i\in \mathcal{S}^t} p_i \Delta^t_i$.
            \STATE Server updates global model $x^{t} = \serveropt(x^{t-1}, -\Delta^t, \eta_s, t)$.
        \ENDFOR
        \end{algorithmic}
        \caption{FedOpt framework}
        \label{alg:fedopt}
    \end{algorithm}
\end{figure*}

We consider the following standard optimization formulation of federated training. We seek to find model parameters $w$ that solve the problem,
\begin{equation}
    \min_{w \in \mathbb{R}^d} f(w) := \sum_{i=1}^m p_i F_i(w)
\end{equation}
where $m$ is the total number of clients, the function $F_i$ measures the average loss of a model with parameters $w$ on the $i$th client's training data, and $p_i > 0$ is the weight given to client $i$. Usually $p_i$ is taken to be proportional to the number of samples at client $i$ so that the optimization problem gives equal weight to all training samples. 
The goal is to find a model that fits all clients' data well on (weighted) average. In FL, only client $i$ can evaluate $F_i$ and its gradient.

All of the methods we consider in this study can be expressed in the general \fedopt framework introduced in~\citet{adaptive-fl-optimization}; see~Algorithm~\ref{alg:fedopt}. At round $t$, the server sends its last model $x^{t-1}$ to a cohort of clients. Each client in the cohort performs $E$ epochs of local training starting from $x^{t-1}$ using \clientopt with client learning rate $\eta_c$, producing a local model $y_i^E$. Then each client communicates the difference $\Delta_i^t$ between their local model and the server model, where $\Delta_i^t := x^{t-1} - y_i^E$. The server computes a weighted average $\Delta^t$ of the client updates (line~9 in Alg.~\ref{alg:fedopt}) and updates its own model via $x_{t+1} = \serveropt(x_t, \Delta_t, \eta_s, t)$, where $\serveropt(x_t, \Delta_t, \eta_s, t)$ is a first-order optimizer, $\eta_s$ is the server learning rate, and $t$ is the round number. 

% \textbf{Gradient Diversity.}
% Gradient diversity quantifies the degree in which individual client updates are different from each other. 
%     We refer to the following ratio as gradient diversity:
%     \[
%     \Delta_S = \frac{\sum_{i=1}^m || \Delta_i ||^2}{|| \sum_{i=1}^m \Delta_i^2 ||}
%     \]

% We say that $\Delta_S$ is a measure of gradient diversity, since it is large when the inner products between the client updates taken with respect to other client data points are small. In particular, gradient diversity is large when the client updates are almost orthogonal and when gradient diversity is small then the client updates are pointing in similar direction. 

% \todo{Add definition of gradient Diversity}

% % \textbf{Cosine Similarity}
% \todo{Do we need to add definition for cosine similarity?}



==> [ICLR] Where to begin_/recommendations.tex <==
\section{Recommendations}
\label{sec:rec}
In this work, we study the effects of pre-training on federated optimization methods. Our results inform the following recommendations: 

1. When evaluating FL algorithms, researchers should experiment with both pre-trained (if available) and random weights, as the initialization can clearly impact the relative performance of different methods, and both initialization schemes may be relevant to practice.

2. When deploying FL to a production environment, using adaptive server optimizers such as \fedadam together with \sgd at the client is a simple and competitive approach when it is possible to start from a pre-trained model. 
    
3. When there is public data to pre-train a model, the impact of heterogeneity can be reduced. Thus, when focusing on heterogeneity, it may be worth considering whether or not proxy data is available for pre-training to motivate the application considered.

% might be more productive for the research community to focus on problems that pre-trained models cannot improve (e.g., FL-powered recommendation systems or semi-supervised learning).
% \mike{Not sure we want to specifically call out recommendation systems or other applications in the paper. We can add something if reviewers ask.}


==> [ICLR] Where to begin_/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
\textbf{Transfer learning.} Model initialization can significantly impact training and final performance. Previous work studying the loss landscape of deep networks observed significant differences between the landscape around a random initialization and the landscape later in training. In particular, later in training, the loss can be much more ``well-behaved'' \citep{hao_vis, frankle_early, frankle_linear}. Fine-tuning from pre-trained models is common practice in natural language processing and computer vision, yielding strong performance on many tasks \citep{gpt2, vit, devlin2018bert, he2019rethinking}.

\textbf{Federated Optimization.} While a significant amount of research focused on various aspects of FL, including communication-efficiency \cite{google-fedavg}, data and systems heterogeneity \cite{fedprox, fednova}, and faster convergence rate \cite{}. Nearly all previous work in this field neglect the importance of initialization. In our work, we study the impact of initialization on federated optimization in the cross-device setting. We defer the interested reader to surveys of \citet{fl-survey} and \citet{fl_field_guide} for additional background.

\textbf{Pre-training in Federated Learning.} Few studies have investigated pre-trained models in federated learning, including \citet{pillutla2022federated, gldv2_fed, zhao2018federated, lin2021fednlp, stremmel2021pretraining, tan2022federated}. While \citet{zhao2018federated} found pre-training does not alleviate the effect of heterogeneity, \citet{tan2022federated} focuses on effectively learning from pre-trained models, and \citet{chen2022pre, weller2022pretrained, chen2022pre} focused on synthetically partitioned data and proposed pre-training methods with synthetic data. Our work fills a gap by comparing random initialization and pre-training, which other studies \cite{pillutla2022federated, gldv2_fed, lin2021fednlp, stremmel2021pretraining} did not address. We systematically investigate both forms of heterogeneity and evaluate 15 SOTA federated optimization algorithms across visual and language tasks. Our study offers theoretical and empirical evidence supporting the benefits of pre-training in FL

% % \label{sec:related_transfer_learning}
% \textbf{Transfer learning.} It is well-known that model initialization can have a significant impact on training and final performance. Previous work studying the loss landscape of deep networks observed that there are significant differences between the landscape around a random initialization and the landscape later in training. In particular, later in training the loss can be much more ``well-behaved'' \citep{hao_vis, frankle_early, frankle_linear}. Fine-tuning from pre-trained models is common practice in natural language processing and computer vision, yielding strong performance on many tasks \citep{gpt2, vit, devlin2018bert, he2019rethinking}.

% % \label{sec:related_federated_transfer_learning}
% \textbf{Federated transfer learning.} Federated transfer learning --- as studied in \citet{ftl, sharma2019secure, ftl_hetro} --- aims to address scenarios where parties share only a partial overlap in the user space or the feature space, and leverages existing transfer learning techniques \citep{weiss2016survey} to build models collaboratively. Partitioning by examples is usually relevant in cross-silo FL when a single company cannot centralize their data due to legal constraints, or when organizations with similar objectives want to collaboratively improve their models~\cite{fl-survey}. In this paper, we focus the scenario where a model is pre-trained at the (centralized) server on public proxy data and then fine-tuned via federated training. We focus primarily on the the large-scale cross-device setting where data partitioning among millions of clients is infeasible, and more generally where stateful methods (those maintaining distinct state about each client) is infeasible. 

% % \label{sec:related_joint_learning}
% \textbf{Joint federated-centralized learning.} There is a line of work on training a model with FL while mixing in data from a centralized dataset \cite{joint_fl, hard2022production} to address the challenge where the federated dataset lacks labeled negative examples. In this paper, we focus on the setting where training takes place in two phases: first, a model is pre-trained on public dataset at the server, and then it is further trained on client data via FL.
% \john{Maybe can we remove this paragraph}

% % \label{sec:related_federated_op}
% \textbf{Federated Optimization.} Significant attention has been paid towards developing federated optimization techniques. Such work has focused on various aspects, including communication-efficiency \cite{google-fedavg}, as well as data and systems heterogeneity \cite{fedprox, fednova}. We defer the interested reader to surveys of \citet{fl-survey} and \citet{fl_field_guide} for additional background. Nearly all previous work in this field neglect the importance of initialization. In our work, we study the impact of initialization on federated optimization in the cross-device setting.  

% Some effort has been made to standardize evaluation, e.g., by introducing benchmark datasets and evaluation protocols~\cite{caldas2018leaf,lai2021fedscale}. Several recommendations are made in the \citet[Section~4]{fl_field_guide} for evaluating and comparing methods, covering topics such as how to form reasonable data splits in FL for tuning learning rates (server and client). However, across nearly all of the literature little attention has been paid to how the model is initialized.

% % \label{sec:related_pre-training} 
% \textbf{Pre-training in Federated Learning.} Very few works have studied pre-trained models in federated learning \cite{pillutla2022federated, gldv2_fed, zhao2018federated, lin2021fednlp, stremmel2021pretraining}.  \citet{zhao2018federated} study pre-training as a mechanism to remedy the accuracy drop compared to centralized training due to heterogeneity in FL. However, they find that using a pre-trained initialization does not help the accuracy drop. In our work, pre-training can close the accuracy gap between centralized and federated training. \citet{pillutla2022federated, gldv2_fed, lin2021fednlp, stremmel2021pretraining} experimented with pre-trained models but did not study the difference between random initialization and pre-training, which is the focus of this work. 

% In concurrent and independent works, \citet{chen2022pre, weller2022pretrained} find that pre-training closes the accuracy gap between \fedavg and centralized learning under non-IID data. \citet{chen2022pre} hypothesize that pre-training makes global aggregation more stable and proposes a method to pre-train with synthetic data. In our work, we systematically study both forms of heterogeneity, data-induced and system-induced. We also find that pre-training can change how federated optimization algorithms behave. 


==> [ICLR] Where to begin_/results.tex <==
\section{The Impact of Pre-Training in FL}
\label{sec:results}
In this section, we illustrate the benefits of pre-training in the federated setting and how pre-training can impact federated optimization algorithms behavior.

% While pre-training unsurprisingly speeds up convergence, the reason for the speedup is less clear in the setting of FL with data heterogeneity. In this section, we illustrate the benefits of pre-training in the federated setting and show that initialization can impact how federated optimization algorithms behave.

\begin{figure*}[t]
     \centering
     \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/so_pre_ran.pdf}
     \end{minipage}
    \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/so_charlm_ran_pre.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.25\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/reddit_ran_pre.pdf}
     \end{minipage}
      \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/cifar_pre_ran.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/cifar_resnet_ran_pre.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.25\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/femnist_pre_ran.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.25\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/femnist_resnet_ran_pre.pdf}
     \end{minipage}
     \caption{While prior works ignore the importance of initialization, using pre-trained models should be the first step for any practical deployment to save on communication bandwidth and achieve high model accuracy. This figure shows the advantage of using a pre-trained model for four tasks. For Stack Overflow and Reddit, we use DistilGPT2. For CIFAR-10 and FEMNIST, we use SqueezeNet. }
     \label{fig:pretrained_vs_random}
\end{figure*}

\textbf{Pre-training changes the ranking of federated optimization algorithms.} 
If one sorts federated optimization methods based on their performance when starting from a random initialization, the order is substantially different from when using a pre-trained initialization. We focus on nine combinations of \serveropt and \clientopt, only using local update methods for \clientopt and excluding full-batch gradient descent. We show the change in performance in Figure \ref{fig:ranking}.

First, observe that the span of final accuracies is much smaller when starting from a pre-trained model. Second, all methods starting with pre-trained models achieve a better accuracy after the same number of steps compared to random models. Lastly, observe that the order of methods changes depending on the initialization. Although no particular method dominates across all workloads in Figure~\ref{fig:ranking},  \fedadam with SGD for \clientopt performs consistently well when starting from a pre-trained model, especially on the two larger language modeling workloads, Stack Overflow and Reddit, and so we focus on studying \fedadam-SGD below.
\begin{wrapfigure}{R}{0.4\textwidth}
     \centering
     \includegraphics[width=0.4\textwidth]{figures/epochs.pdf}
     \caption{The accuracy for CIFAR-10 using ResNet-18 with increasing number of local epochs.}
     \label{fig:more_local_steps}
\end{wrapfigure}

% \label{sec:faster_convergence}
\textbf{Faster convergence to better accuracy when starting from a pre-trained model.}
Figure~\ref{fig:pretrained_vs_random} shows that, as one would hope, when starting from a pre-trained model, it is possible to achieve much better accuracy after a fixed number of steps than when starting federated training from a random initialization. Note that the initial accuracy is not always substantially higher than a random initialization (See Table \ref{fig:initial_loss}). 

\textbf{Pre-training closes the accuracy gap between non-IID and IID.} 
We study how pre-training and data heterogeneity affect convergence without system heterogeneity by fixing the number of local epochs to $E_i = 1$. We compare \fedadam-\sgd under IID and Non-IID data splits. 
In Figure~\ref{fig:data_heterogeneity}, we report the average accuracy for FedAdam \citep{adaptive-fl-optimization} on the four datasets. As expected, randomly initialized models perform much worse than their pre-trained counterparts, and IID partitions yield better quality than non-IID. Surprisingly, the gap between models trained on IID data and models trained on non-IID data is significantly smaller when starting with pre-trained weights. Moreover, pre-training reduces the negative effects of data heterogeneity (i.e., client drift). As a result, we observe that (see \Cref{fig:more_local_steps}) when training from a pre-trained model, increasing the number of local updates does not degrade the final accuracy, in contrast to training from a random model

\textbf{\fedadam \gd is as effective as \fedadam \sgd with pre-training.} The seminal work of \citet{google-fedavg} shows that taking local SGD steps before server averaging reduces communication by 10-100$\times$ compared to taking a full batch gradient step. To understand how pre-training impacts this comparison, we compare \fedadam with \sgd and \fedadam with \gd. While local \sgd can reduce communication, the saving is much less when the models are initialized with pre-trained weights compared to random weights. Figure \ref{fig:local_steps} in the Appendix shows that with pre-trained initialization, using \gd at the client can yield almost the same result as taking local SGD steps.


% To measure how data heterogeneity and pre-training impact model accuracy, we compare performance under IID and Non-IID data splits using the approaches described above.  In Figure \ref{fig:data_heterogeneity}, we report the average accuracy for FedAdam \citep{adaptive-fl-optimization} across four datasets. As expected, random initialization models perform much worse than their pre-trained counterparts, and IID partitions yield better quality than non-IID. However, the surprising result is that the gap between FL with IID data and FL with non-IID data is significantly smaller when using pre-trained models. Figure~\ref{fig:data_heterogeneity} shows a smaller drop in accuracy for pre-trained models (0.6\% for FEMINIST, 3.9\% for Stack Overflow, 7.5\% for CIFAR-10, and 1.92\% for Reddit). Interestingly, pre-training on publicly available datasets such as Imagenet demonstrates robust results for various FL tasks. For example, FEMINIST and Imagenet are two very different datasets. FEMINIST consists of black and white digits and characters, while Imagenet contains colored images. Despite this, pre-training on Imagenet closes the accuracy from data heterogeneity. On both CIFAR-10 and Stack Overflow, MineLite outperforms other methods in the random initialization setting indicated by the dotted line moving up the parallel plots. 
% \john{Discuss figure 7 and figure 6, the effect of hetrogenity is less so we can take more local epochs and full batch GD can perform well. }

\begin{figure*}[t]
     \centering
    % \begin{minipage}[t]{\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figures/accurac_drop.pdf}
    %  \end{minipage}
     \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/CIFAR-10.pdf}
     \end{minipage}
    %  \hspace{1em}
     \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/Stack_Overflow.pdf}
     \end{minipage}
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/FEMNIST.pdf}
     \end{minipage}
    \begin{minipage}[t]{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/Reddit.pdf}
     \end{minipage}
     \caption{The average accuracy on 3 different seeds for \fedadam trained on IID and non-IID data. For CIFAR-10 Non-IID, we generate 100 non-IID clients using a Dirichlet(0.1). For other three datasets, we use the natural non-IID client partitions.}
     \label{fig:data_heterogeneity}
\end{figure*}

\textbf{Pre-training reduces the impact of system heterogeneity.} To study the impact of pre-training on system heterogeneity, we follow the setup described in \citep{fedprox,fednova}. 
We sample 30\% of clients uniformly at random, and client $i$ performs $E_i$ local epochs where $E_i \sim U(1, 5)$ while the remaining 70\% of the clients perform $E_i = 1$ epochs; this models the setting where clients have different processing capabilities and they perform as much work as they can within a given time limit. Figure~\ref{fig:system_heterogeneity} shows that \fedadam-\sgd consistently outperforms other methods specifically designed for system heterogeneity (\nova, \proximal, \mimelite) when starting from a pre-trained model. Apparently using an adaptive optimizer at the server is sufficient to correct for the negative effects of systems heterogeneity when starting from a pre-trained model. On the other hand, when starting from a random initialization, optimizers specifically designed for system heterogeneity (i.e., \textsc{FedNova}) outperform \sgd (Figure \ref{fig:system_heterogeneity} right).  Moreover, the accuracy gap between algorithms is more pronounced in the random initialization setting, whereas in the pre-trained setting, all algorithms converge to more similar accuracies. Our results suggest that pre-training may reduce the need for algorithms that try to correct system heterogeneity. 

% \label{sec:system_hetro}
% Figure \ref{fig:system_heterogeneity} displays the average accuracy for \fedavg, \fedavgm and \fedadam as \serveropt. For \clientopt, we use \sgd, two other local optimizers designed specifically to handle system heterogeneity, \proximal~\citep{fedprox} and normalized averaging (\nova)~\citep{fednova}, and one targeting client drift \mimelite \citep{karimireddy2021mime}.

\begin{figure*}[t]
     \centering
     \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/cifar_pre_sys.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/cifar_ran_sys.pdf}
     \end{minipage}
      \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/femnist_pre_sys.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/femnist_ran_sys.pdf}
     \end{minipage}
     \caption{System heterogeneity results comparing FedAvg, FedAvgM and FedAdam with various client optimizers. We simulate system heterogeneity by randomly select 30\% of clients per round to perform time-varying local epochs $E_i \sim U(1, 5)$, the same approach as in \cite{fednova}. FedProx and FedNova correspond to FedAvg with Proximal client optimizer and normalized averaging (\nova), respectively. We repeat each experiment for 3 different seeds and report the average.}
     \label{fig:system_heterogeneity}
\end{figure*}

% \todo{Need a better way to present Table \ref{tab:system_heterogeneity}}


% \mike{Does the same conclusion hold for MimeLite?} 
% \john{Mention about the much bigger gap between different algorithms in random init}

\section{Understanding Why Pre-training Helps Federated Optimization}
\label{sec:why_pretrain}

While pre-training unsurprisingly speeds up convergence, the reason for the speedup is less apparent. In this section, we examine why pre-training is beneficial to federated learning. 
% \label{sec:cosine}

\begin{figure*}[t]
     \centering
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/train_loss_cifar.pdf}
     \end{minipage}
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/dis_from_init.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/eval_accuracy.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.32\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/gradient_diversity.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/cosine.pdf}
     \end{minipage}
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/dis_to_final.pdf}
     \end{minipage}
     \caption{Training and gradient statistics of a Resnet18 on CIFAR-10 with Dirichlet distribution with parameter 0.1. Top row: Train loss of global model; train accuracy of global model; evaluation accuracy of global model; evaluation loss of global model. Bottom row: Gradient diversity of client updates; cosine similarity between client updates; L2 distance of server weights from their final values at the end of training.}
     \label{fig:gradident_stats}
\end{figure*}

\textbf{Pre-training helps align client updates.} To better understand why pre-training alleviates the heterogeneity challenge, we first investigate the gradient diversity of the updates received from different clients. 
We adopt the notion introduced in~\citet{gradient-diversity}, adapted here to apply to client updates $\Delta_i$ (whereas \citet{gradient-diversity} focus specifically on gradients $g_i$):
\[
\operatorname{GradientDiversity}(\{\Delta_i \colon i \in \mathcal{S}^t\}) = \frac{\sum_{i \in \mathcal{S}^t} || \Delta_i ||^2}{|| \sum_{i \in \mathcal{S}^t} \Delta_i^2 ||}.
\]

In Figure \ref{fig:gradident_stats}, we plot the gradient diversity of client updates $\Delta_i$ at each round for \fedadam. In the pre-trained setting, client updates have significantly lower gradient diversity (see the bottom left plot in Figure \ref{fig:gradident_stats}). This suggests that when starting from a pre-trained model, the client local model changes are more similar to each other. On the other hand, clients local model changes from randomly initialized weights are almost orthogonal, suffering more from the client drift problem. In addition, when looking at the cosine similarity of consecutive aggregated update vectors in time (bottom middle), we see that consecutive updates point more consistently in a similar direction at the beginning of training when starting from a pre-trained model.

From the top middle and bottom right plots in Figure \ref{fig:gradident_stats}, we see that the pre-trained model starts closer to the final result. We also examine the largest eigenvalue of the Hessian matrix (i.e., local Lipshitz constant or smoothness) at the beginning of training, a larger value of which suggests a harder-to-optimizer loss surface. To compute the Hessian matrix, We examine the largest eigenvalue of the Hessian matrix at initialization, round 0, using Power Iteration from PyHessian by \cite{yao2020pyhessian}. In \Cref{fig:hessian_datasets}, one can observe that pre-trained models always lead to smaller eigenvalues on different datasets.

% This observation helps to understanding why pre-training narrows the accuracy gap between FL on non-IID and IID data. Figure \ref{fig:gradident_stats} (bottom right and bottom middle) demonstrates that the client updates from pre-trained weights travel in a \textit{"straighter"} direction compared to those from random weights. On the other hand,  client updates from randomly initialized weights are almost orthogonal. By taking the average of many orthogonal updates as the pseudo-gradient, the server model takes longer to reach its final model. This explains Figure \ref{fig:gradident_stats} (top right), as the pre-trained model weights move faster to their final values.



% \john{does anyone know how to combine figure \ref{fig:more_local_steps} and Table \ref{fig:hessian_datasets} into two columns side-by-side to save space?}\jianyu{Does `minipage' work here?}


% \label{sec:local_steps}

% \subsection{Pre-training allows for more local steps to speed up convergence.}
% \label{sec:more_local_steps}


% \subsection{Pre-training improves the smoothness of the local loss functions. }
% \label{sec:hessian}
 

\begin{table}
\begin{center}
\begin{tabular}{l l l l l } 
    \toprule
     ~ & CIFAR-10 & FEMNIST & Stack Overflow & Reddit \\
     \midrule
      Pre-trained & 661.99   & 26.29  & 151.05  & 647.19 \\
      Random      & 4843.13  & 355.51 & 185.02 & 1309.68 \\
     \bottomrule
\end{tabular}
\end{center}
\caption{The top eigenvalue of the Hessian matrix for each dataset between the pre-trained and random initialized models.}
\label{fig:hessian_datasets}
\end{table}

\begin{table*}
\centering
\begin{tabular}{llllllllll} 
\toprule
               & CIFAR-10       &             & FEMNIST &             &  \\ 
\midrule
               & Squeezenet 1.0         & ResNet-18 & Squeeze 1.0  & ResNet-18 &  \\
Pre-trained      & 2.71           & 1.07        & 3.99    & 6.58        &  \\ 
Random & 1.90           & 1.11        & 4.31    & 4.17        &  \\
\bottomrule \toprule
               & Stack Overflow &             & Reddit  &             &  \\ 
\midrule
               & CharLM         & DistilGPT2 & CharLM  & DistilGPT2 &  \\
Pre-trained     & 6.78           & 4.93        & 5.15    & 6.34        &  \\
Random         & 7.71           & 9.82        & 8.61    & 9.99        &  \\
\bottomrule
\end{tabular}\caption{Loss at beginning of training for various model architectures and datasets. The initial loss of the pretrained model is not always lower than that of a random initialization.}
\label{fig:initial_loss}
\end{table*}

\textbf{Initial loss for pre-trained versus random models.}
% \label{sec:initial_loss}
Table \ref{fig:initial_loss} shows that pre-training does not always lead to lower initial loss. For Squeezenet 1.0 on CIFAR-10 and ResNet-18 on FEMNIST, the initial loss of the randomly initialized models are lower pre-trained models. However, pre-trained model still converges faster as illustrated in Figure \ref{fig:pretrained_vs_random}.

==> [ICLR] Where to begin_/theory.tex <==
\textbf{Connection to theory.} Here, we present the existing optimization theory for \fedavg and discuss how pre-training helps to improve the model convergence. Following the formulation in Section 3, suppose that there are total $m$ clients, jointly optimizing a global objective function $f(w) = \sum_{i=1}^m p_i F_i(w)$, and that each client's local loss function $F_i(w)$ is $L$-Lipschitz smooth. For ease of presentation, we assume that all clients participate in training and perform $K$ local SGD updates at each round. Then, under standard assumptions, one can show that after $R$ communication rounds, the expected gradient norm satisfies (see Theorem~V in \cite{SCAFFOLD}):
\begin{equation}
\E \norm{ \nabla f(\bar{x}^R) }^2 \le \mathcal{O}\left(\frac{\sqrt{F}}{\sqrt{RKm}} + \frac{F^{2/3}\zeta^{2/3}}{R^{2/3}} \right), \label{eqn:error_bnd}
\end{equation}
where $\bar{w}^R$ represents a weighted sampled model from all previous rounds, $\zeta$ is a measure of data heterogeneity, and $F =f(x^0) - f^*$ denotes the gap between the initial loss value and the optimal loss value. 

In addition, in order for \fedavg to achieve the $\mathcal{O}(1/\sqrt{RKm})$ asymptotic convergence rate, previous works~\citep{fl_field_guide,woodworth2020minibatch,SCAFFOLD,wang2021cooperative} showed that the number of local updates $K$ should be upper bounded as follows:
\begin{align}
    K \leq \mathcal{O}\left( \frac{R^{1/3}}{F^{1/3}\zeta^{4/3}m} \right).
\end{align}
Clearly, if $F$ becomes smaller starting from a pre-trained model, one can use a larger number of local updates. This corroborates our empirical observations in \Cref{fig:more_local_steps}.

When starting from a pre-trained model, the initial gap $F$ is sometimes reduced, as observed in \Cref{fig:initial_loss}. As a result, the optimization error upper bound (\ref{eqn:error_bnd}) will be smaller, i.e., we get better worst-case performance. However a lower initial loss is not always observed in our experiments, so this does not fully explain our observations, suggesting that we may need to re-think the convergence theory of local update methods.

==> intro_old.tex <==
\section{Introduction}
\label{sec:intro}
\emph{Federated learning} (FL) has emerged as a popular distributed machine learning paradigm for privately training a shared model across many participants while the training data never leaves the participant devices. Our focus in this work is on understanding the impact of model initialization on federated learning.

In cross-device FL~\citep{fl-survey}, the primary setting considered in this paper, a large number of client devices (possibly on the order of hundreds of millions) participate in training, which is coordinated by a server. It is impractical for all devices to participate at every step of training; instead, FL usually proceeds in rounds and a small subset of available devices participate in each round. Each device possesses a local dataset, and the data at different devices follow different distributions, leading to the \emph{data heterogeneity} challenge~\citep{fl-survey}. Moreover, devices communicate with the server over low-bandwidth, high-latency links, making communication overhead a major performance factor.

The predominant approach to federated training builds on local update methods such as \textsc{FedAvg}~\citep{google-fedavg}, where a device performs several local updates (e.g., one epoch of SGD on their local training set) before transmitting an update to the server. Although this reduces communication overhead, it can also exacerbate the data heterogeneity problem. Several approaches have been proposed to address this challenge~\citep{fedprox,fedavgm,adaptive-fl-optimization,fednova,SCAFFOLD,karimireddy2021mime,zhang2021fedpd,acar2021feddyn}.

\textbf{This paper empirically investigates the impact of model initialization on federated optimization methods.} Previous empirical evaluations of FL methods nearly always start federated training from a randomly initialized model. Transfer learning from pre-trained models has become common practice in natural language processing~\cite{gpt2,devlin2018bert} and computer vision~\cite{he2019rethinking,vit}, yielding state-of-the-art results on many tasks and enabling faster model convergence in the centralized setting. However, the impact of starting federated training from a pre-trained model has not been carefully studied, even though in many practical applications of FL there is public proxy data available for pre-training at the server.

\paragraph{Contributions.} In this work we consider the question:
\begin{center}
    \it How does model initialization (random, or pre-trained) impact \\the behavior of federated optimization methods?
\end{center}
Towards answering this question, we perform an extensive empirical study, comparing 15 variations of federated optimization methods on four commonly-used FL benchmark datasets. Our study reveals four key findings:
\begin{enumerate}
    % \item Federated optimization methods behave differently when initialized randomly versus from pre-trained weights (Section~\ref{sec:results_ranking}). \mike{Definitely rewrite this to be more specific; currently too vague or just not so surprising.}
    % \item \mike{Shouldn't the first point be about optimizers designed to address heterogeneity not being the best when starting from a pre-trained initialization?}
    \item Optimizers designed to address heterogeneity are not as effective when starting from pre-trained initialization. 
    % the effect of system and data heterogeneity is less of a problem when initializing federated optimization from a pre-trained solution.  \mike{Again, elaborate on exactly what ``less of a problem'' means here.}

    \item Starting from a pre-trained solution can close the gap between training on IID and non-IID data (Section~\ref{sec:results}). Moreover, the simple \sgd at the client outperforms more complex local-update methods in the pre-trained setting.
    
    \item Towards starting to explain this phenomenon, we observe that inter-device gradient/update diversity is higher for random initialized model at the beginning of training, and inter-device cosine similarity is higher when starting from a pre-trained model. (Section~\ref{sec:why_pretrain})
    
    \item When starting from a pre-trained solution, the client can afford to take more local steps to save on communications without hurting final accuracy. \john{Reword this finding}
    
    % Surprisingly, full-batch gradient descent, without any local steps, achieves performance competitive with other SoTA local-update methods from a pre-trained initialization. 

    % \mike{Maybe add something specifically about the performance of local-update methods vs those that don't use local updates (FedGD, ...)?}

\end{enumerate}
Our experiments also confirm what one might expect, that initializing FL with a pre-trained model can increase final model accuracy and reduce the number of rounds required to achieve a target accuracy, thereby saving communications and reducing the overall training time. This is evident in Figure~1 across several datasets (hyperparameters were tuned separately for each dataset--initialization pair; see Section~\ref{sec:experiments} for details of the experimental setup). 

\begin{figure*}[t]
     \centering
     \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/so_pre_ran.pdf}
     \end{minipage}
    \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/so_charlm_ran_pre.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.25\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/reddit_ran_pre.pdf}
     \end{minipage}
      \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/cifar_pre_ran.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/cifar_resnet_ran_pre.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.25\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/femnist_pre_ran.pdf}
     \end{minipage}
     \begin{minipage}[t]{0.25\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/femnist_resnet_ran_pre.pdf}
     \end{minipage}
     \caption{While prior works ignore the importance of initialization, using pre-trained models should be the first step for any practical deployment to save on communication bandwidth and achieve high model accuracy. This figure shows the advantage of using a pre-trained model for four tasks. For Stack Overflow and Reddit, we use DistilGPT2 and CharLM. For CIFAR-10 and FEMNIST, we use SqueezeNet and ResNet18. }
     \label{fig:pretrained_vs_random}
\end{figure*}

Our findings are reproducible using the open-source federated learning framework FLSim~\cite{flsim}. Informed by these findings, we conclude by presenting several recommendations for future research on federated optimization.
